Temporal Extrapolation of Elastic Seismic Wave Propagation in Layered Media Using Neural Operators

Temporal prediction of seismic velocity fields beyond the time interval represented in training remains challenging for neural operator models. This study develops a coupled neural operator framework for stress-conditioned temporal prediction in layered elastic media. A time-integrator-embedded Deep Operator Network (TI-DeepONet) advances the velocity field through an embedded fourth-order Runge-Kutta (RK4) scheme, while a Fourier Neural Operator (FNO) learns a residual correction to the predicted spatial field. The two components are trained jointly in a predictor-corrector configuration. Prediction is initialized with reference velocity fields at the first two time levels and proceeds autoregressively, with reference stress fields and prescribed excitation supplied throughout rollout, including beyond the training interval. Four cases consider horizontally polarized shear (SH) waves in four-layer soil columns with fixed total depths of 50 and 280 m, excited by third-order Gaussian-derivative (DOG3) wavelets with central frequencies between 0.5 and 6 Hz. Layer thicknesses and shear-wave velocities vary across profiles. Evaluations on test profiles extend beyond the training interval by up to twice its duration. The predictions reproduce principal velocity arrivals and depth-dependent response patterns, with accuracy varying across profiles. Across the four cases, mean peak-normalized root-mean-square errors (NRMSEs) range from 0.53% to 2.31% over the full evaluation windows and from 0.61% to 2.82% over the extrapolation intervals. Both metrics use each profile's peak absolute reference velocity over the full evaluation window as the normalizer. These results demonstrate temporal velocity prediction under reference-stress conditioning for the tested configurations; autonomous continuation of the coupled velocity-stress wavefield remains to be established.

==> latexmkrc <==
# This shows how to use the xr package with latexmk.
# John Collins 2023-03-29
#
# The xr package ("a system for eXternal References") is used by a document
# to make references to sections, equations, etc in other external
# documents. 
# The definitions in this file enable latexmk to apply latexmk to
# automatically update an external document whenever its .tex file changes,
# so that the references in the main document stay up to date.

# Notes:
#    1. This version is defined to put the files from the compilations of
#       the external documents into a defined subdirectory, to segregate
#       potentially many generated files from the main document
#       directories. 
#    2. But for latexmk's custom dependency mechanism to be used, as here,
#       the aux file from compilation of a subdocument must be generated in
#       the same directory as the corresponding source .tex file.  So the
#       .aux file is copied.
#    3. It is assumed that the external documents are to be compiled by
#       pdflatex.  This can be changed, of course, by changing the '-pdf'
#       option given to the invoked latexmk to whatever is needed.
#    4. An ideal implementation would also ensure that recompilation of an
#       external document also happens whenever any of its other source
#       files changes.  But this is not done in the present version, and
#       would probably entail either the use of internal latexmk variables
#       or extra enhancements to latexmk.
#    5. The code uses subroutines copy and fileparse that are loaded by
#       latexmk from the Perl packages File::Copy and File::Basename.
#    6. It also uses some not-yet-documented features of latexmk: an array
#       variable @file_not_found and subroutines popd, pushd, and
#       rdb_add_generated. 


#--------------------
# Configurable choices for compilation of external documents

# Subdirectory for output files from compilation of external documents:
$sub_doc_output = 'output-subdoc';

# Options to supply to latexmk for compilation of external documents:
@sub_doc_options = ();

push @sub_doc_options, '-pdf'; # Use pdflatex for compilation of external documents.
# Replace '-pdf' by '-pdfdvi', 'pdfxe', or 'pdflua' if needed.

#--------------------

# Add a pattern for xr's log-file message about missing files to latexmk's
# list.  Latexmk's variable @file_not_found is not yet documented.
# This line isn't necessary for v. 4.80 or later of latexmk.
push @file_not_found, '^No file\\s*(.+)\s*$';

add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
sub makeexternaldocument {
    if ( $root_filename ne $_[0] )  {
        my ($base_name, $path) = fileparse( $_[0] );
        pushd $path;
        my $return = system "latexmk",
                            @sub_doc_options,
                            "-aux-directory=$sub_doc_output",
                            "-output-directory=$sub_doc_output",
                            $base_name;
        if ( ($sub_doc_output ne '') && ($sub_doc_output ne '.') ) {
               # In this case, .aux file generated by pdflatex isn't in same
               # directory as the .tex file.
               # Therefore:
               # 1. Actual generated aux file must be listed as produced by this
               #    rule, so that latexmk deals with dependencies correctly.
               #    (Problem to overcome: If $sub_dir_output is same as $aux_dir
               #    for the main document, xr may read the .aux file in the
               #    aux_dir rather than the one the cus dep is assumed by latexmk
               #    to produce, which is in the same directory as the .tex source
               #    file for this custom dependency.)
               #    Use not-yet-documented latexmk subroutine rdb_add_generated
               #    to do this:
               # 2. A copy of the .aux file must be in same directory as .tex file
               #    to satisfy latexmk's definition of a custom dependency.
             rdb_add_generated( "$sub_doc_output/$base_name.aux" );
             copy "$sub_doc_output/$base_name.aux", ".";
        }
        popd;
        return $return;
   }
}
